AI Assisted Experiment Control and Calibration

Final report for the AI Assisted Experiment Control and Calibration project. This project integrated AI/ML into the controls and calibration of a production detector system in the GlueX spectrometer, a large scale Nuclear Physics detector in experimental Hall-D at Jefferson Lab. The AI/ML model predicted calibration constants for a Central Drift Chamber using environmental information available prior to taking the data. The device controls were then automatically adjusted so that the calibration values needed for post-processing of the data were much more stable and quicker to determine. Integration into a production system required guardrails and policy choices to ensure safety of the equipment and the data quality. The project sought to apply similar technology to other detectors. Those efforts are also described here. This documents many of the details of the project.

==> Sections/FcalSimML/FcalSimML_original.tex <==
\subsubsection{FCAL Simulated Machine Learning} \label{sec:sim}
\hl{needs an introduction}

Here we discuss  progress in an ongoing simulation study   to determine what limitations there are in extracting gains from LED pulse amplitudes. This will hopefully allow us to determine a good model architecture to use with the real data.

The ADC readout amplitude, A, is modeled as a function of block number (b) and time (t) by the following equation:
\begin{equation}
        A(b,t) = g({b,t)^{-1} \cdot \omega(b) \cdot \alpha(t) \cdot R(b,t) + \epsilon(b,t)
\end{equation}
where $g$ is the PMT gain,
\begin{equation}
    g(b,t) = A_1\sin(\omega_1 t + \phi_1) + A_2\sin(\omega_2 t + \phi_2)
\end{equation}
and where the optical coupling constant, $\omega_{b,t}$, is sampled from a normal distribution:
\begin{equation}
    \omega(b,t)=\mathcal{N}(\mu, \sigma^2)
\end{equation}
 with $\mu=1$ and $\sigma=0.1$. 
The amplitude of the LED pulser is defined as
\begin{equation}
    
\end{equation}

$R(b,t)$ is the radiation damage for each block, and $\epsilon$ is an additional noise parameter. For the purposes of this study, the radiation factor R is set equal to one. 
Fig. \ref{fig:gf} shows an example of the factors that go into calculating the LED pulse amplitude at each time step without the addition of stochastic noise.

%this figure needs to be redone
\begin{figure}[htb]
    \centering
    \includegraphics[width=1\linewidth]{Sections/FcalSimML/gf.png}
    \caption{Gain Factors}
    \label{fig:gf}
\end{figure}

%The LED pulser amplitude $\alpha$ is modeled as a piecewise linear function that reverses direction when the amplitude reaches a given threshold above or below one or randomly with a given probability. The distribution of true FCAL gain calibration values for all blocks are shown in Fig. \ref{}.

%The LED pulser amplitude $\alpha$ is modeled as piece wise line segments that reverse direction once they achieve an amplitude that is specified as a given percentage above or below the nominal value of unity, but also randomly with a given probability. 


%\paragraph{PMT Gain} The distribution of true FCAL gain calibration values are shown in Fig. \hl{we hope to add a true FCAL distribution early in the document}, with most values being close to one. 
%Thus, for the simulation, the PMT gain $g$ for each block is modeled as a superposition of two sine functions of arbitrary frequency, phase, and amplitude relationship centered around one.


\paragraph{Stochastic Noise} System noise $\epsilon$ is modeled as  Zero Mean Gaussian White Noise (ZMGWN), possibly block dependent such that when

\begin{equation}\label{eqn:epsilonx}
    \epsilon \leftarrow N(0,x)
\end{equation}

we say that we are modeling at an $100 \cdot x$ percent noise level.


\paragraph{Feature Engineering} Mimicking the experimental setup described in Section \ref{sec:fcal}, the ADC Readout amplitude $A$, shown in Fig. \ref{fig:gf}, is the only input data available.
Modeling efforts using Eq. \ref{eqn:bigA} to directly solve for the PMT gain $g$ yielded inferior results. 
Thus, the following precursor feature engineering method was implemented as described here.

\paragraph{}Using equation (\ref{eqn:bigA}) with $\omega$ and $R$ constant for each block we can write:

\begin{equation}\label{eqn:alpha_hat}
    \hat{\alpha}_t = mean_b(A_{b,t})
\end{equation}

as our estimate of the LED pulser amplitude $\alpha$ where the mean is taken across blocks for each discrete time step and here we are treating  the PMT gain $g^{-1}$  as a {\it nuisance parameter}.  Fig. \ref{fig:ae10} shows an example  of this model:

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Sections/FcalSimML/alpha_es_10.png}
    \caption{Estimated LED pulser Amplitude at 10\% Noise}
    \label{fig:ae10}
\end{figure}


It is then possible to estimate  the Optical Coupling constant $\omega_b$  for each block as:

%\begin{equation}\label{eqn:sclfctr0}
%    \hat{\omega}^{-1}_b = \frac{mean_t(\hat{\alpha})}{mean_t(A_{b})}
%\end{equation}


\begin{equation}\label{eqn:sclfctr}
    \hat{\omega}_b = \frac{mean_t(A_{b})}{mean_t(\hat{\alpha})}
\end{equation}

where the mean is taken across the time index. Finally, we define the average amplitude for the PMT gain $g$ as

%\begin{equation}\label{eqn:gb_est0}
%    \hat{(g^{-1})}_{b,t} = \hat{\omega}^{-1}_b \cdot \frac{A_{b,t}}{\hat{\alpha}_t}
%\end{equation}


\begin{equation}\label{eqn:gb_est}
    \hat{g_{b,t}} = \hat{\omega}_b \cdot \frac{\hat{\alpha}_t}{A_{b,t}}
\end{equation}

 It then remains to see if machine learning techniques can improve this first model if it is used as the sole feature input.  Some examples  of this AA model:

\begin{figure}[H]

\begin{subfigure}{0.5\textwidth}
\includegraphics[width=0.9\linewidth, height=5cm]{Sections/FcalSimML/aa0.png} 
\caption{AA  and Actual PMT Gain at 0\% Noise}
\label{fig:subim1}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=0.9\linewidth, height=5cm]{Sections/FcalSimML/aa5.png}
\caption{AA  and Actual PMT Gain at 5\% Noise}
\label{fig:subim2}
\end{subfigure}

\caption{AA  and Actual PMT Gain}
\label{fig:image2}
\end{figure}


\begin{figure}[H]

\begin{subfigure}{0.5\textwidth}
\includegraphics[width=0.9\linewidth, height=5cm]{Sections/FcalSimML/aa10.png} 
\caption{AA  at 10\% Noise}
\label{fig:subim1a}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=0.9\linewidth, height=5cm]{Sections/FcalSimML/AAvsg5.png}
\caption{AA vs Actual PMT Gain at 5\% Noise}
\label{fig:subim2a}
\end{subfigure}

\caption{AA  and Actual PMT Gain}
\label{fig:image3}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{Sections/FcalSimML/aa0.png}
    \caption{AA  at 0\% Noise}
    \label{fig:aa0}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{Sections/FcalSimML/aa5.png}
    \caption{AA  at 5\% Noise}
    \label{fig:aa3}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{Sections/FcalSimML/aa10.png}
    \caption{AA at 10\% Noise}
    \label{fig:aa10}
\end{figure}

\begin{figure}[H]
    \centering
    \includegraphics[width=0.7\linewidth]{Sections/FcalSimML/AAvsg5.png}
    \caption{AA vs Actual PMT Gain at 5\% Noise}
    \label{fig:AAvsg5}
\end{figure}

Fig \ref{fig:AAvsg5} shows that at 5\% noise level the AA calculation, while a  noisy fit to the PMT gain (red line), nonetheless demonstrates no systematic bias in its figure, the centroid (black line) of which faithfully represents the deterministic PMT signal.  Other noise levels demonstrate this as well.  It is then expected that  ML modeling will denoise this basic result into a final model.

\paragraph{Machine Learning}We use the LHS of Eq. \ref{eqn:gb_est} as the lone feature input to predictive models for Generalized Linear Model (GLM), Three Layer Perceptron (TLP), Random Forest (RF), and Long Short-Term Memory (LSTM) a type of recurrent neural network.

\paragraph{}Training for each model used an 80\%/20\% split for training/prediction without shuffling to preserve the time sequence sense of the data.  Models were evaluated at noise levels from 1\% to 5\% with the exception of the AA and LSTM models which were extended to 10\%. Results were also obtained for LSTM for series histories of 1 to 50 time units across all noise levels.  One hundred samples (trained solutions) were drawn for each noise level for models AA, GLM, TLP, RF , and 25 samples were drawn for LSTM across both noise levels and history window depths.  Figs. \ref{fig:all-mae} and \ref{fig:all_mxmae} depict these results.

\paragraph{Results} We use the primary metric of Mean Absolute Error (MAE) for model performance comparisons, where MAE is determined across the time index for the 20\% validation portion of the data for each sample.  As indicated by Fig. \ref{fig:all-mae}, mean performance degrades as the noise level increases for all models, where by {\it mean performance} we mean the mean of the sample MAEs for each noise level and history window depth for LSTM.  As a practical matter, models GLM, TLP, and RF were evaluated up to a maximum noise level of 5\% as fits above that level were deemed unacceptable for those models.  Observed performance for models GLM, TLP, and RF were nearly indistinguishable.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Sections/FcalSimML/all-mae.png}
    \caption{All Models MAE}
    \label{fig:all-mae}
\end{figure}

\paragraph{}If we establish a notional acceptance criteria of 1\% mean MAE, that is to say {\it average performance}, we see that the AA, GLM, TLP, and RF models just graze acceptability up to about 2\% noise whereas the LSTM(50) is acceptable out to about the 9\% noise level, where LSTM(50) is the LSTM model for history depth of 50 time units.  Table \ref{tab:fcal_model_results} summarizes these results for mean MAE and standard error of mean MAE.


\paragraph{}If instead the metric is  1\% mean Maximum MAE, or {\it worst-case performance}, we see (Fig. \ref{fig:all_mxmae}) that only the LSTM(50) model is acceptable and only for the 1\% noise level.


\begin{figure}[H]
    \centering
    \includegraphics[width=0.8\linewidth]{Sections/FcalSimML/all-mxmae.png}
    \caption{All Models Max MAE}
    \label{fig:all_mxmae}
\end{figure}

\paragraph{} Fig. \ref{fig:lstm9} shows a typical performance curve for LSTM.  Here at 9\% noise level, best average performance can be achieved at a history window depth of about 25 whereas best worst-case performance requires a history window depth of about 40.

\begin{figure}[H]
    \centering
    \includegraphics[width=0.9\linewidth]{Sections/FcalSimML/lstm9.png}
    \caption{LSTM at 9\% Noise}
    \label{fig:lstm9}
\end{figure}


\begin{table}[H]
\small
\centering
\caption{MAE (\%) Results from Modeling Competition for PMT Gain.}
\begin{tabular}{lllllllllll}
\hline
\textbf{Model} & \textbf{AA} & & \textbf{GLM} & & \textbf{TLP} & & \textbf{RF} & & \textbf{L(50)} & \\
\hline
Noise & Mean & StdErr & Mean & StdErr & Mean & StdErr & Mean & StdErr & Mean & StdErr \\
\hline
1\% & 0.83 & 0.005 & 0.7 & 0.003 & 0.68 & 0.003 & 0.73 & 0.003 & 0.34 & 0.01 \\
2\% & 1.28 & 0.006 & 1.07   & 0.004 & 1.07   & 0.005 & 1.09   & 0.005 & 0.51 & 0.021 \\
3\% & 1.79 & 0.008 & 1.39 & 0.006 & 1.39 & 0.005 & 1.42 & 0.007 & 0.64 & 0.017 \\
4\% & 2.31 & 0.01 & 1.61 & 0.007 & 1.65 & 0.007 & 1.65 & 0.006 & 0.71 & 0.021 \\
5\% & 2.87 & 0.016 & 1.78 & 0.006 & 1.81 & 0.006 & 1.81 & 0.008 & 0.78 & 0.022 \\
6\% & 3.39 & 0.014 &  - &  - &  - &  - &  - &  - & 0.89 & 0.029 \\
7\% & 3.97 & 0.019 &  - &  - &  - &  - &  - &  - & 0.98 & 0.029 \\
8\% & 4.53 & 0.019 &  - &  - &  - &  - &  - &  - & 1.09 & 0.029 \\
9\% & 5.09 & 0.025 &  - &  - &  - &  - &  - &  - & 1.1 & 0.041 \\
10\% & 5.65 & 0.028 &  - &  - &  - &  - &  - &  - & 1.24 & 0.048 \\
\hline
\end{tabular}

\label{tab:fcal_model_results}
\end{table}


